Neural Enhanced Belief Propagation for Cooperative Localization

Location-aware networks will introduce innovative services and applications for modern convenience, applied ocean sciences, and public safety. In this paper, we establish a hybrid method for model-based and data-driven inference. We consider a cooperative localization (CL) scenario where the mobile agents in a wireless network aim to localize themselves by performing pairwise observations with other agents and by exchanging location information. A traditional method for distributed CL in large agent networks is belief propagation (BP) which is completely model-based and is known to suffer from providing inconsistent (overconfident) estimates. The proposed approach addresses these limitations by complementing BP with learned information provided by a graph neural network (GNN). We demonstrate numerically that our method can improve estimation accuracy and avoid overconfident beliefs, while its computational complexity remains comparable to BP. Notably, more consistent beliefs are obtained by not explicitly addressing overconfidence in the loss function used for training of the GNN.

==> LatexInclusion/catechism.tex <==
%----------------------------------------------------------------------------------------%
%                                       C a t e c h i s m                                         %
%----------------------------------------------------------------------------------------%
\section*{Research Paper Catechism\footnote{Adapted from George Heilmeier.}} 

\vspace{0.5cm} 

\be\itemsep3ex

\item What is the big picture? What is the problem and why is it hard?
	\bi
	\item[$\diamond$] The Big Picture: \BigPicture
	\item[$\diamond$] The Problem/Difficulty: \ProblemDifficulty
%	\item[$\diamond$] The Difficulty:
	\ei

\item What are the classical approaches? What is the state-of-the-art and what are the deficiencies?
	\bi
	\item[$\diamond$] Classical Approaches: \ClassicApproach
	\item[$\diamond$] The State-of-the-Art and Deficiencies:  \SOADeficiency
	\item[ ] \mysubsubnote{This is where you make a literature review. Articulate the deficiencies and shortcomings of previous work. Provide references (you can use the first three alphabets of the authors' last names and year, similar to the convention in our database).}
	\ei
	
\item What are the fundamental questions relevant to the problem? How answering to these questions can impact the design, architecture, and operation?
	\bi
	\item[$\circ$] \FundamentalQ
	\item[$\circ$] \EnablingA 
	\item[ ] \mysubsubnote{This is where you persuade the reader that these are fundamental questions, and the answers to these questions will have game-changing impacts.}
	\ei	

\item What are the goals of our paper?
	\bi
	\item[$\diamond$] The Goals:
	\item[ ] \mysubsubnote{Describe the goals at a high level; this should correlate with high-level contributions in Question 6.}
	\ei
		\be
		\item[$\circ$] \Goals 
		\ee		

\item What are we advocating; what is the new technical idea; what is our new view; what is our credence? Why we can succeed now? 
	\bi
	\item[$\diamond$] Advocacy, Idea, View, and Credence:
	\item[ ] \mysubsubnote{For example:}
		\be
		\item[$\circ$] \Advocacy 
		\ee
	\item[$\diamond$] Reasons for Success:
	\item[ ] \mysubsubnote{For example:}
		\be
		\item[$\circ$] \ReasonSuccess 
		\ee
	\ei

\item What are the high-level contributions of our  paper? What are the key contributions of our paper? 
	\bi
	\item[$\diamond$] High-Level Contributions: \HLContribution
	\item[ ] \mysubsubnote{Describe what we do at a high level; this should address the goal that we set out in Question 4; for example:}
		\be
		\item[$\circ$] In this paper, \ldots
		\ee
	\item[$\diamond$] Key Contributions:
	\item[ ] \mysubsubnote{Provide a bulletized list (usually 3-5 bullets, equal number of lines per bullets); for example:}
		\be
		\item[$\circ$] \KeyContribution
		\ee
	\ei


\item Which are the methodologies (analysis, simulation, experimentation, heterogeneous approach) used in this paper? How is the approach verified; how are the results confirmed?
	\bi
	\item[$\diamond$] The Methodologies: Inference on graphs, graph theory, graph neural networks
	\item[$\diamond$] The Verification: 
	\ei
	
\item What are the new vision/perspective we provide? What are the lessons learned?
	\bi
	\item[$\diamond$] The New Vision/Perspective: \ConclusiveVision
	\item[$\diamond$] The Lessons Learned/Surprising Results: \ConclusiveLesson
	\ei

\item What is the impact; what are the benefits or merits of the results to a broader community?
	\bi
	\item[$\diamond$] The Impact/Benefit: \Benefit
	\item[ ] \mysubsubnote{Think of strong conclusions for the paper when answering them}
	\ei


\item Where the known results appear in the paper?
	\bi
	\item[$\diamond$] Disclosures: Scalable probabilistic data association with so called ``point-targets'' based on the sum-product algorithm was proposed previously. Parts of the original technique is used as an element of the scalable data association algorithm for extended targets presented in Section \ref{sec:scalableSPA}.
	\item[ ] \mysubsubnote{Identify where known results appear in the paper (point to specific section numbers before the paper is written; point to specific section, page, line, equation numbers, etc. after the paper is written).}
	\item[$\diamond$] Sources: Probabilistic data association with point-targets based on the sum-product algorithm \cite{WilLau:J14,MeyBraWilHla:J17,MeyKroWilLauHlaBraWin:J18}.
	\item[ ] \mysubsubnote{Identify what are the sources (provide reference, section, page, line, equation numbers, etc. of the sources).}
	\ei

\item What are the key references?
\bi
	\item[ ] \mysubsubnote{List the key references that we used to develop this paper (rather than the references for the state-of-the-art).}
	
	Message Passing \cite{KscFreLoe:01,YedFreWei:05,KolFri:B09}; \acp{gnn} \cite{GorMonSca:05, YooLiaXioZhaFetUrtZemPit:19, SatWel:20}; \ac{cl} \cite{WymLieWin:09}
	
% 	MOT (``point target''): \cite{BarWilTia:B11,Mah:B07,MeyKroWilLauHlaBraWin:J18}; EOT \cite{HabThaKirGriWak:C11,HamSveSanSor:J12,HabThaThaMalKir:J13
% 	,SchReuWan:C15,CorCar:J18,GenVivBraSolAmi:J15,VivBra:J16,GraOrg:J12,LunGraOrg:J13,BeaReuGraVoVoSch:J16,GraFatSve:J17}: 
\ei

\ee

